Discovering novel quantum dynamics with NISQ simulators

Major technological advances of the past century are rooted in our understanding of quantum physics in the non-interacting limit. A central challenge today is to understand the behavior of complex quantum many-body systems, where interactions play an essential role. About four decades ago, Richard Feynman proposed using controllable quantum systems to efficiently simulate complex physics and chemistry problems, envisioning quantum orreries, highly tunable quantum devices built to emulate less understood quantum systems. Here we ask whether quantum simulators have already uncovered new physical phenomena-and, if so, in which areas and with what impact. We find that, in several notable instances, they have advanced our understanding of many-body quantum dynamics. Although many of these insights could in principle have been obtained theoretically or numerically, they were nevertheless first achieved using quantum processors. While a broad landscape of problems beyond non-equilibrium dynamics still awaits exploration, it is encouraging that quantum simulators are already beginning to challenge and refine our conventional wisdom.

==> macros.tex <==
\def\({\left(}
\def\){\right)}

\def\bra#1{\mathinner{\langle{#1}|}}
\def\ket#1{\mathinner{|{#1}\rangle}}
\def\braket#1#2{\mathinner{\langle{#1}|#2 \rangle}}

\def\avg#1{\mathinner{\langle{#1} \rangle}}

\def\Id{{\rm Id}}
\def\CZ{{\rm CZ}}
\def\CR{{\rm CR}}
\def\T{{\rm T}}
\def\X{{\rm X}}
\def\Y{{\rm Y}}
\def\Z{{\rm Z}}
\def\H{{\rm H}}
\def\A{{\cal A}}
\def\IQC{{\rm IQC}}
\def\bP{{\mathbb P}}
\def\cL{{\mathcal L}}

\def\u#1{^{(#1)}}
\def\c#1{{\mathcal #1}}

%\def\tr{{\rm tr}\,}
\newcommand{\tr}{\operatorname{tr}}

\newtheorem{conjecture}{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}


% Figures. Example usage:
% \quickfig{\columnwidth}{my_image}{This is the caption}{fig:my_fig}
\DeclareRobustCommand{\quickfig}[4]{
\begin{figure}
\begin{centering}
\includegraphics[width=#1]{#2}
\par\end{centering}
\caption{#3}
\label{#4}
\end{figure}
}

\DeclareRobustCommand{\quickwidefig}[4]{
\begin{figure*}[h]
\begin{centering}
\includegraphics[width=#1]{#2}
\par\end{centering}
\caption{#3}
\label{#4}
\end{figure*}
}
